Interpreting DeepStack-Style Vision-Language Models: Do Input or Deeper-Layer Visual Tokens Drive Answers?

DeepStack-style vision-language models inject visual tokens at the language-model input (main entry) and deeper decoder layers (later entries), yet same-image visual question-answering accuracy cannot reveal how trained models divide work between them. We therefore feed main and later mismatched versions of one image, differing in an object's attribute (e.g., color), visual quality (undegraded versus desaturated, blurred, or downsampled), or both. Under a single-object color conflict on photographs, original DeepStack follows the later entries, whereas Qwen3-VL-8B and 32B follow main. When main receives a desaturated synthetic image while later keeps an undegraded recolored object, later shifts the log-probability margin between the two colors more strongly than with undegraded main across all four tested models (including Granite Vision). Whether later can also recover lost accuracy, however, depends sharply on the model: when blur at both entries costs both Qwen models 50 percentage points on a synthetic visual task, keeping later undegraded recovers 48 points in Qwen3-VL-32B but only 8 in Qwen3-VL-8B. Unlike conflict dominance, these recovery patterns identify which entry each model can zero out with little GQA attribute loss. Although DeepStack follows later under conflict, either entry suffices on GQA attributes (at most 3.45 points lost when zeroed), letting split inference (transmitting compressed visual features) send only main at higher precision and cut bytes by 49% at comparable accuracy versus compressing all entries. Thus, an entry's role cannot be inferred from the architecture or same-image accuracy, and must be diagnosed per checkpoint before pruning or compressing features.

==> table_style.tex <==
\RequirePackage{colortbl}
\RequirePackage{tabularx}
\definecolor{DSTableHeader}{HTML}{EBEBEE}
\definecolor{DSTableAccent}{HTML}{EAEDFB}
\newlength{\DSCompactTableWidth}

\makeatletter
\newdimen\DS@ov \DS@ov=.25pt
\newcount\DS@colidx
\newcount\DS@ncolbuild
\def\DS@ncols{0}
\newif\ifDS@record
\newif\ifDS@inmc
\def\DS@lastsep{0}
\def\DS@mclastsep{0}
\def\CT@setup{%
  \global\advance\DS@colidx\@ne
  \@tempdimb\z@
  \@tempdimc\z@
  \ifnum\DS@colidx<\DS@ncols\relax\@tempdimc\DS@ov\fi
  \ifDS@inmc
    \global\DS@inmcfalse
    \ifnum\DS@mclastsep=\@ne\@tempdimc\DS@ov\fi
  \else
    \ifnum\DS@lastsep=\@ne\@tempdimc\DS@ov\fi
  \fi
  \def\CT@color{%
    \global\let\CT@do@color\CT@@do@color
    \color}}
\@ifundefined{CT@row@color}{\global\let\CT@row@color\relax}{}
\newif\ifDS@aftercell
\protected\def\DS@colsep{%
  \ifx\CT@row@color\relax
    \hskip\col@sep
  \else
    {\let\CT@color\color\CT@row@color
     \ifDS@aftercell
       \leaders\vrule\hskip\col@sep
     \else
       \kern-\DS@ov\leaders\vrule\hskip\dimexpr\col@sep+2\DS@ov\relax\kern-\DS@ov
     \fi}%
  \fi}
\let\DS@orig@classz\@classz
\def\@classz{\global\advance\DS@ncolbuild\@ne\DS@orig@classz}
\let\DS@orig@mkpream\@mkpream
\def\@mkpream#1{\global\DS@ncolbuild\z@\DS@orig@mkpream{#1}%
  \ifnum\@lastchclass=\z@\def\DS@tempa{1}\else
    \ifnum\@lastchclass=\tw@\def\DS@tempa{1}\else\def\DS@tempa{0}\fi\fi
  \ifDS@record
    \global\DS@recordfalse
    \xdef\DS@ncols{\the\DS@ncolbuild}\global\let\DS@lastsep\DS@tempa
  \else
    \global\let\DS@mclastsep\DS@tempa
  \fi}
\let\DS@CT@start\CT@start
\def\CT@start{\DS@CT@start
  \edef\DS@colstate{\global\DS@colidx\the\DS@colidx\relax
    \gdef\noexpand\DS@ncols{\DS@ncols}\gdef\noexpand\DS@lastsep{\DS@lastsep}}%
  \global\DS@colidx\z@\global\DS@recordtrue}
\let\DS@CT@end\CT@end
\def\CT@end{\DS@CT@end\DS@colstate}
\let\DS@orig@multicolumn\multicolumn
\long\def\multicolumn#1#2#3{\DS@orig@multicolumn{#1}{#2}{\DS@mcspan{#1}#3}}
\def\DS@mcspan#1{\global\advance\DS@colidx\numexpr#1-1\relax\global\DS@inmctrue}
\let\DS@CT@@do@color\CT@@do@color
\def\CT@@do@color{\aftergroup\DS@aftercelltrue\DS@CT@@do@color}
\def\@acol{\@addtopreamble{\DS@colsep}}
\setlength{\aboverulesep}{\z@}
\setlength{\belowrulesep}{\z@}
\newdimen\DS@rowpad \DS@rowpad=.6pt
\newif\ifDS@intable
\newif\ifDS@padded
\def\DS@tablepad{\DS@intabletrue\setlength{\extrarowheight}{\DS@rowpad}}
\AddToHook{env/table/begin}{\DS@tablepad}
\AddToHook{env/table*/begin}{\DS@tablepad}
\def\DS@padstrut{%
  \ifDS@intable\ifDS@padded\else
    \DS@paddedtrue
    \setbox\strutbox\hbox{\vrule\@height\ht\strutbox\@depth\dimexpr\dp\strutbox+\DS@rowpad\relax\@width\z@}%
  \fi\fi}
\AddToHook{env/tabular/begin}{\DS@padstrut}
\AddToHook{env/tabularx/begin}{\DS@padstrut}
\global\let\DS@lastrowcolor\relax
\CT@everycr{\noalign{%
  \global\let\DS@lastrowcolor\CT@row@color
  \global\let\CT@row@color\relax
  \global\DS@colidx\z@}\the\everycr}
\let\DS@orig@BTendrule\@BTendrule
\def\@BTendrule{\global\let\DS@lastrowcolor\relax\DS@orig@BTendrule}
\def\DS@rowdone{%
  \ifx\DS@lastrowcolor\relax\else
    \ifdim\lastskip=\z@
      \vskip-\DS@ov
      {\let\CT@color\color\CT@row@color\hrule\@height\DS@ov\@depth\DS@ov}%
      \vskip-\DS@ov
    \fi
  \fi
  \ifnum0=`{\fi}}
\def\CT@rowc{%
  \@ifnextchar[\CT@rowd\DS@rowdone}
\def\CT@rowe[#1][#2]{%
  \@tempdimb#1%
  \@tempdimc#2%
  \xdef\CT@row@color{%
    \expandafter\noexpand\CT@row@color
    \@tempdimb\the\@tempdimb
    \@tempdimc\the\@tempdimc
    \relax}%
  \DS@rowdone}

\definecolor{DSInterval}{HTML}{7C7C82}
\def\DS@akey{none}
\newcommand\DSalign[1]{\def\DS@akey{#1}}
\newsavebox\DS@boxL
\newsavebox\DS@boxR
\newsavebox\DS@boxI
\def\DS@cisize{%
  \ifdim\f@size pt>9.5pt \fontsize{9}{10.5}\selectfont
  \else\ifdim\f@size pt>8.5pt \fontsize{8}{9.5}\selectfont
  \else\ifdim\f@size pt>7.5pt \fontsize{7}{8.5}\selectfont
  \else \fontsize{6}{7}\selectfont\fi\fi\fi}
\newcommand\DSci[1]{{\DS@cisize\color{DSInterval}$#1$}}
\def\DS@split#1.#2.#3\DS@nil{\def\DS@int{#1}\def\DS@frac{#2}}
\def\DS@key{\edef\DS@ckey{\DS@akey/\the\numexpr\DS@colidx+1\relax}}
\def\DS@rec#1#2#3#4{\DS@max{DS@L@#1}{#2}\DS@max{DS@R@#1}{#3}\DS@max{DS@I@#1}{#4}}
\def\DS@max#1#2{\@ifundefined{#1}{\global\@namedef{#1}{#2}}%
  {\ifnum#2>\csname#1\endcsname\relax\global\@namedef{#1}{#2}\fi}}
\def\DS@note{\immediate\write\@auxout{\string\DS@rec{\DS@ckey}%
  {\number\wd\DS@boxL}{\number\wd\DS@boxR}{\number\wd\DS@boxI}}}
\def\DS@width#1{\ifcsname DS@#1@\DS@ckey\endcsname
  \csname DS@#1@\DS@ckey\endcsname sp\else\wd\csname DS@box#1\endcsname\fi}
\def\DS@number#1#2{%
  \DS@split#2..\DS@nil
  \sbox\DS@boxL{#1\DS@int#1}%
  \sbox\DS@boxR{\ifx\DS@frac\@empty\else#1.\DS@frac#1\fi}}
\def\DS@value{\makebox[\DS@width{L}][r]{\usebox\DS@boxL}\makebox[\DS@width{R}][l]{\usebox\DS@boxR}}
\newcommand\DSv[2]{\DS@key\DS@number${#1}%
  \if\relax\detokenize{#2}\relax\else
    \sbox\DS@boxR{\usebox\DS@boxR\hspace{.3em}\DSci{#2}}\fi
  \sbox\DS@boxI{}\DS@note\DS@value}
\newcommand\DSn[1]{\DS@key\DS@number{}{#1}\sbox\DS@boxI{}\DS@note\DS@value}
\newcommand\DSat[2]{\DS@key\sbox\DS@boxL{#1}\sbox\DS@boxR{#2}\sbox\DS@boxI{}\DS@note\DS@value}
\newdimen\DS@stackpad \DS@stackpad=1.5pt
\newcommand\DSstack[2]{\DS@key\DS@number${#1}\sbox\DS@boxI{\DSci{#2}}\DS@note
  \begin{tabular}[c]{@{}c@{}}%
    \rule{\z@}{\dimexpr\ht\@arstrutbox+\DS@stackpad}\DS@value\\[-\DS@stackpad]
    \rule[-\dimexpr\dp\@arstrutbox+\DS@stackpad]{\z@}{\z@}%
    \makebox[\DS@width{I}][c]{\usebox\DS@boxI}%
  \end{tabular}}
\makeatother

